Multilingual Large Language Models: A Systematic Survey

This paper provides a comprehensive survey of the latest research on multilingual large language models (MLLMs). MLLMs not only are able to understand and generate language across linguistic boundaries, but also represent an important advancement in artificial intelligence. We first discuss the architecture and pre-training objectives of MLLMs, highlighting the key components and methodologies that contribute to their multilingual capabilities. We then discuss the construction of multilingual pre-training and alignment datasets, underscoring the importance of data quality and diversity in enhancing MLLM performance. An important focus of this survey is on the evaluation of MLLMs. We present a detailed taxonomy and roadmap covering the assessment of MLLMs' cross-lingual knowledge, reasoning, alignment with human values, safety, interpretability and specialized applications. Specifically, we extensively discuss multilingual evaluation benchmarks and datasets, and explore the use of LLMs themselves as multilingual evaluators. To enhance MLLMs from black to white boxes, we also address the interpretability of multilingual capabilities, cross-lingual transfer and language bias within these models. Finally, we provide a comprehensive review of real-world applications of MLLMs across diverse domains, including biology, medicine, computer science, mathematics and law. We showcase how these models have driven innovation and improvements in these specialized fields while also highlighting the challenges and opportunities in deploying MLLMs within diverse language communities and application scenarios. We listed the paper related in this survey and publicly available at https://github.com/tjunlp-lab/Awesome-Multilingual-LLMs-Papers.

==> taxonomies/alignment_evaluation.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=hidden-pink!80, text=black, align=center,font=\tiny,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
    font=\fontsize{5}{5}\selectfont
]
\begin{figure*}[t!]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=center,
                font=\tiny,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=center,
                text centered,
                minimum width=2em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=6em,font=\tiny,}{},
            where level=2{text width=12em,font=\tiny,}{},
            where level=3{text width=12em,font=\tiny,}{},
            where level=4{text width=10em,font=\tiny,}{},
            [
                \textbf{Alignment Evaluation}
                [
                    Ethics and Morality 
                    [
                        Expert-defined Ethics and Morality
                        [
                            \citet{DBLP:conf/acl/JohnsonG18} \\ eMFD \citep{hopp2021extended} \\ \citet{DBLP:conf/emnlp/ForbesHSSC20} \\       \citet{DBLP:conf/emnlp/ForbesHSSC20} \\
                            TrustGPT \citep{DBLP:journals/corr/abs-2306-11507} \\
                            \citet{DBLP:conf/iclr/HendrycksBBC0SS21} \\
                            % \citep{Situated Reasoning about Norms, Intents, Actions, and their Consequences}
                            , leaf
                        ]
                    ]
                    [
                        Crowdsourced Ethics and Morality
                        [
                            \citet{DBLP:journals/corr/abs-2101-07664} \\
                            \citet{DBLP:conf/nips/JinLAKSSMTS22}
                            , leaf
                        ]
                    ]
                    [  
                        AI-assisted Ethics and Morality
                        [
                            \citet{DBLP:journals/corr/abs-2307-14324} \\
                            PROSOCIALDIALOG \citep{DBLP:conf/emnlp/0002YJLKKCS22} \\
                            \citet{DBLP:conf/acl/ZiemsYWHY22}
                            , leaf
                        ]
                    ]
                    [
                        Hybrid Ethics and Morality
                        [
                            SCRUPLES \citep{DBLP:conf/aaai/LourieBC21} 
                            , leaf
                        ]
                    ]
                ]
                [
                    Bias
                    [
                        Societal Bias in Downstream Tasks
                        [
                            Coreference Resolution
                            [
                                Winogender \citep{DBLP:conf/naacl/RudingerNLD18} \\ 
                                WinoBias \citep{DBLP:conf/naacl/ZhaoWYOC18} \\ \citet{DBLP:conf/aaaiss/Levesque11} \\ \citet{DBLP:journals/tacl/WebsterRAB18} \\ 
                                GICOREF \citep{DBLP:conf/acl/CaoD20} 
                                % \citep{DBLP:conf/acl/BlodgettLOSW20}
                                , leaf
                            ]
                        ]
                        [
                            Machine Translation
                            [
                                % \citep{DBLP:conf/emnlp/Alvarez-MelisJ17} \\ \citep{DBLP:journals/corr/abs-1901-03116} \\ 
                                WinoMT \citep{DBLP:conf/acl/StanovskySZ19} \\ \citet{DBLP:journals/corr/abs-2104-07838} 
                                , leaf
                            ]
                        ]
                        [
                            Natural Language Inference
                            [
                                \citet{DBLP:conf/aaai/DevLPS20} \\ \citet{DBLP:conf/emnlp/PenningtonSM14} 
                                , leaf
                            ]
                        ]
                        [
                            Sentiment Analysis
                            [
                                \citet{DBLP:conf/ijcai/DiazJLPG19} \\ \citet{DBLP:conf/cscw/LazarDBKP17} \\ 
                                EEC \citep{DBLP:conf/starsem/KiritchenkoM18} 
                                , leaf
                            ]
                        ]
                        [
                            Relation Extraction
                            [
                                WikiGenderBias \citep{DBLP:conf/acl/GautSTHQEZMBCW20}
                                , leaf
                            ]
                        ]
                        [
                            Implicit Hate Speech Detection
                            [
                                \citet{DBLP:conf/aies/DixonLSTV18} \\ \citet{DBLP:conf/www/BorkanDSTV19} \\ \citet{do2019jigsaw} \\ \citet{DBLP:conf/acl/HutchinsonPDWZD20} \\ \citet{DBLP:conf/acl/SapGQJSC20} \\ \citet{DBLP:conf/emnlp/BreitfellerAJT19} \\
                                Latent Hatred \citep{DBLP:conf/emnlp/ElSheriefZMASCY21} \\
                                DynaHate \citep{DBLP:conf/acl/VidgenTWK20} \\
                                TOXIGEN \citep{DBLP:conf/acl/HartvigsenGPSRK22} \\
                                CDail-Bias \citep{DBLP:journals/corr/abs-2202-08011} \\
                                CORGI-PM \citep{DBLP:journals/corr/abs-2301-00395} \\
                                HateCheck \citep{DBLP:conf/acl/RottgerV0WMP20}
                                , leaf
                            ]
                        ]
                    ]
                    [
                        Societal Bias in LLMs
                        [
                            StereoSet \citep{DBLP:conf/acl/NadeemBR20} \\
                            CrowS-Pairs \citep{DBLP:conf/emnlp/NangiaVBB20} \\ \citet{DBLP:journals/corr/abs-2301-09211} \\ 
                            BOLD \citep{DBLP:conf/fat/DhamalaSKKPCG21} \\  
                            \citet{DBLP:journals/corr/abs-2104-08728} \\
                            HolisticBias \citep{DBLP:conf/emnlp/SmithHKPW22} \\ 
                            \citet{DBLP:journals/corr/abs-2305-13198} \\
                            Unqover \citep{DBLP:journals/corr/abs-2010-02428} \\
                            BBQ \citep{DBLP:conf/acl/ParrishCNPPTHB22} \\
                            CBBQ \citep{DBLP:journals/corr/abs-2306-16244} \\
                            \citet{DBLP:conf/acl/ZhaoMHCA20} \\
                            FairLex \citep{DBLP:conf/acl/ChalkidisP0TSS22}
                            , leaf
                        ]
                    ]
                ]
                [
                    Toxicity
                    [
                        Toxicity Identification and Classification
                        [
                            OLID \citep{DBLP:conf/naacl/ZampieriMNRFK19} \\ 
                            SOLID \citep{DBLP:conf/acl/RosenthalAKZN21} \\
                            OLID-BR \citep{trajano2023olid} \\ 
                            KODOLI \citep{DBLP:conf/eacl/ParkKLKLLL23} \\
                            % \citep{DBLP:conf/naacl/ZampieriMNRFK19} \\ \citep{DBLP:conf/acl/RosenthalAKZN21} \\
                            % \citep{trajano2023olid} \\ 
                            % \citep{DBLP:conf/eacl/ParkKLKLLL23} \\
                            % \citep{DBLP:journals/corr/abs-2205-12390}
                            , leaf
                        ]
                    ]
                    [
                        Toxicity Evaluation
                        [
                            RealToxicityPrompts \citep{DBLP:conf/emnlp/GehmanGSCS20} \\ \citet{DBLP:journals/corr/abs-2304-05335} \\
                            HarmfulQ \citep{DBLP:conf/acl/Shaikh0HBY23} \\ 
                            PerspectiveAPI \citep{DBLP:conf/kdd/Lees0TSGMV22}
                            % \citep{DBLP:conf/emnlp/GehmanGSCS20} \\ \citep{DBLP:journals/corr/abs-2304-05335} \\
                            % \citep{DBLP:conf/acl/Shaikh0HBY23} \\ 
                            % \citep{DBLP:conf/kdd/Lees0TSGMV22}
                            , leaf
                        ]
                    ]
                ]
                [
                    Truthfulness
                    [
                        Datasets
                        [
                            Question Answering
                            [
                                NewsQA \citep{DBLP:conf/rep4nlp/TrischlerWYHSBS17} \\
                                SQuAD 2.0 \citep{DBLP:conf/acl/RajpurkarJL18} \\
                                BIG-bench \citep{DBLP:journals/corr/abs-2206-04615} \\
                                SelfAware \citep{DBLP:conf/acl/YinSGWQH23} \\
                                TruthfulQA \citep{DBLP:conf/acl/LinHE22} \\
                                HalluQA \citep{DBLP:journals/corr/abs-2310-03368} \\
                                , leaf
                            ],
                        ]
                        [
                            Dialogue
                            [
                                DialFact \citep{DBLP:conf/acl/GuptaWLX22} \\
                                \citet{DBLP:conf/emnlp/HonovichCANSA21} \\
                                BEGIN \citep{DBLP:journals/tacl/DziriRLR22} \\
                                ConsisTest \citep{lotfi-etal-2022-name} \\
                                , leaf
                            ]
                        ]
                        [
                            Summarization
                            [
                                XSumFaith \citep{DBLP:conf/acl/MaynezNBM20} \\
                                FactCC \citep{DBLP:conf/emnlp/KryscinskiMXS20} \\
                                SummEval \citep{DBLP:journals/tacl/FabbriKMXSR21} \\
                                FRANK \citep{DBLP:conf/naacl/PagnoniBT21} \\
                                SummaC \citep{DBLP:journals/tacl/LabanSBH22} \\
                                \citet{DBLP:conf/acl/WangCL20} \\
                                \citet{DBLP:conf/naacl/GoyalD21} \\
                                \citet{DBLP:conf/acl/CaoDC22} \\
                                CLIFF \citep{DBLP:conf/emnlp/Cao021} \\
                                AggreFact \citep{DBLP:conf/acl/TangGFL0YKRD23} \\
                                PolyTope \citep{DBLP:conf/emnlp/HuangCYBWXZ20} \\
                                , leaf
                            ]
                        ]
                    ]
                    [
                        Methods
                        [
                            NLI-based Methods
                            [
                                \citet{DBLP:conf/acl/WelleckWSC19} \\
                                \citet{lotfi-etal-2022-name} \\
                                \citet{DBLP:conf/acl/FalkeRUDG19} \\
                                \citet{DBLP:journals/tacl/LabanSBH22} \\
                                \citet{DBLP:conf/acl/MaynezNBM20} \\
                                \citet{DBLP:journals/corr/abs-2212-10622} \\
                                \citet{DBLP:conf/naacl/UtamaBMG22} \\
                                \citet{DBLP:conf/acl/RoitFSACDGGHKMG23} \\
                                , leaf
                            ]
                        ]
                        [
                            QAQG-based Methods
                            [
                                FEQA \citep{DBLP:conf/acl/DurmusHD20} \\
                                QAGS \citep{DBLP:conf/acl/WangCL20} \\
                                QuestEval \citep{DBLP:conf/emnlp/ScialomDLPSWG21} \\
                                QAFactEval \citep{DBLP:conf/naacl/FabbriWLX22} \\
                                Q2 \citep{DBLP:conf/emnlp/HonovichCANSA21} \\
                                FaithDial \citep{DBLP:journals/tacl/DziriKMZYPR22} \\
                                \citet{DBLP:conf/acl/DengZH023} \\
                                , leaf
                            ]
                        ]
                        [
                            LLMs-based Methods
                            [
                                FIB \citep{DBLP:conf/acl/TamMZKBR23} \\
                                FacTool \citep{DBLP:journals/corr/abs-2307-13528} \\
                                FActScore \citep{DBLP:journals/corr/abs-2305-14251} \\
                                SelfCheckGPT \citep{DBLP:journals/corr/abs-2303-08896} \\
                                SAPLMA \citep{DBLP:journals/corr/abs-2304-13734} \\
                                \citet{DBLP:journals/tmlr/LinHE22} \\
                                \citet{DBLP:journals/corr/abs-2207-05221} \\
                                , leaf
                            ]
                        ]
                    ]
                ]
            ] 
        \end{forest}
    }
    \caption{Overview of alignment evaluations.}
    \label{fig:alignment_evaluation}
\end{figure*}

==> taxonomies/evaluation_organization.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=hidden-pink!80, text=black, align=center,font=\normalsize,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
]
\begin{figure*}[t!]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=center,
                font=\large,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=center,
                text centered,
                minimum width=5em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=8em,font=\normalsize,}{},
            where level=2{text width=15em,font=\normalsize,}{},
            where level=3{text width=18em,font=\normalsize,}{},
            % where level=4{text width=10em,font=\normalsize,}{},
            [
                \textbf{Evaluation Organization}
                [
                    Benchmarks for \\NLU and NLG
                    [
                        GLUE \citep{DBLP:conf/iclr/WangSMHLB19} \\
                        SuperGLUE \citep{DBLP:conf/nips/WangPNSMHLB19} \\
                        CLUE \citep{DBLP:conf/coling/XuHZLCLXSYYTDLS20} \\
                        DynaBench \citep{DBLP:conf/naacl/KielaBNKGWVPSRM21} \\
                        LongBench \citep{DBLP:journals/corr/abs-2308-14508}
                        , leaf
                    ]
                ]
                [
                    Benchmarks for \\Knowledge and \\Reasoning
                    [
                        MMLU \citep{DBLP:conf/iclr/HendrycksBBZMSS21} \\
                        MMCU \citep{DBLP:journals/corr/abs-2304-12986} \\
                        C-Eval \citep{DBLP:journals/corr/abs-2305-08322} \\
                        AGIEval \citep{DBLP:journals/corr/abs-2304-06364} \\
                        M3KE \citep{DBLP:journals/corr/abs-2305-10263} \\
                        M3Exam \citep{DBLP:journals/corr/abs-2306-05179} \\
                        CMMLU \citep{DBLP:journals/corr/abs-2306-09212} \\
                        LucyEval \citep{DBLP:journals/corr/abs-2308-04823}
                        , leaf
                    ]
                ]
                [
                    Benchmarks for \\Holistic \\Evaluation
                    [
                        Leaderboards
                        [
                            Evaluation Harmness \citep{gao2021framework} \\ HELM \citep{DBLP:journals/corr/abs-2211-09110} \\ BIG-bench \citep{DBLP:journals/corr/abs-2206-04615} \\ CLEVA \citep{DBLP:journals/corr/abs-2308-04813} 
                            , leaf
                        ]
                    ]
                    [
                        Arena
                        [
                            Chatbot Arena \citep{DBLP:journals/corr/abs-2306-05685}
                            , leaf
                        ]
                    ]
                ]
            ] 
        \end{forest}
    }
    \caption{Overview of LLM evaluation organization.}
    \label{fig:evaluations_organization}
\end{figure*}

==> taxonomies/knowledge_and_capability_evaluation.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=hidden-pink!80, text=black, align=center,font=\normalsize,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
]
\begin{figure*}[t!]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=center,
                font=\large,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=center,
                text centered,
                minimum width=5em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=15em,font=\normalsize,}{},
            where level=2{text width=14em,font=\normalsize,}{},
            where level=3{text width=21em,font=\normalsize,}{},
            where level=4{text width=22em,font=\normalsize,}{},
            where level=5{text width=18em,font=\normalsize,}{},
            [
                \textbf{Knowledge and Capability Evaluation}
                [
                    Question Answering
                    [
                        Dataset
                        [
                            SQuAD \citep{DBLP:conf/emnlp/RajpurkarZLL16} \\
                            NarrativeQA \citep{DBLP:journals/tacl/KociskySBDHMG18} \\
                            HotpotQA \citep{DBLP:conf/emnlp/Yang0ZBCSM18} \\
                            CoQA \citep{DBLP:journals/tacl/ReddyCM19} \\
                            DuReader \citep{DBLP:conf/acl/TangL0H0020} \\
                            , leaf
                        ]
                    ]
                    [
                        Evaluation
                        [
                            Natural Questions \citep{DBLP:journals/tacl/KwiatkowskiPRCP19} \\
                            , leaf
                        ]
                    ]
                ]
                [
                    Knowledge Completion
                    [
                        Subject-Relation-Object \\ Triples Prediction
                        [
                            LAMA \citep{DBLP:conf/emnlp/PetroniRRLBWM19} \\
                            KoLA \citep{DBLP:journals/corr/abs-2306-09296} \\
                            WikiFact \citep{DBLP:conf/kdd/GoodrichRLS19} \\
                            , leaf
                        ]
                    ]
                ]
                [
                    Reasoning
                    [
                        Commonsense Reasoning
                        [
                            Datasets
                            [
                                ARC \citep{DBLP:journals/corr/abs-1803-05457} \\
                                QASC \citep{DBLP:conf/aaai/KhotCGJS20} \\
                                MCTACO \citep{DBLP:conf/emnlp/ZhouKNR19} \\
                                TRACIE \citep{DBLP:conf/naacl/ZhouRNKSR21} \\
                                TIMEDIAL \citep{DBLP:conf/acl/QinGUHCF20} \\
                                HellaSWAG \citep{DBLP:conf/acl/ZellersHBFC19} \\
                                PIQA \citep{DBLP:conf/aaai/BiskZLGC20} \\
                                Pep-3k \citep{DBLP:conf/naacl/WangDE18} \\
                                Social IQA \citep{DBLP:conf/emnlp/SapRCBC19} \\
                                CommonsenseQA \citep{DBLP:conf/naacl/TalmorHLB19} \\
                                OpenBookQA \citep{DBLP:conf/emnlp/MihaylovCKS18} \\
                                , leaf
                            ]
                        ]
                        [
                            Empirical Evaluation
                            [
                                \citet{DBLP:journals/corr/abs-2302-04023} \\
                                \citet{DBLP:journals/corr/abs-2303-16421} \\
                                , leaf
                            ]
                        ]
                    ]
                    [
                        Logical Reasoning
                        [
                            Datasets
                            [
                                Natural Language Inference Datasets
                                [
                                    SNLI \citep{DBLP:conf/emnlp/BowmanAPM15} \\
                                    MultiNLI \citep{DBLP:conf/naacl/WilliamsNB18} \\
                                    LogicNLI \citep{DBLP:conf/emnlp/TianLCX0J21} \\
                                    ConTRoL \citep{DBLP:conf/aaai/LiuCL021} \\
                                    MED \citep{DBLP:conf/blackboxnlp/YanakaMBISAB19} \\
                                    HELP \citep{DBLP:conf/starsem/YanakaMBISAB19} \\
                                    ConjNLI \citep{DBLP:conf/emnlp/SahaNB20} \\
                                    TaxiNLI \citep{DBLP:conf/conll/JoshiASC20} \\
                                    , leaf
                                ]
                            ]
                            [
                                Multiple-choice Reading Comprehension Datasets
                                [
                                    ReClor \citep{DBLP:conf/iclr/YuJDF20} \\
                                    LogiQA \citep{DBLP:conf/ijcai/LiuCLHWZ20} \\
                                    LogiQA 2.0 \citep{DBLP:journals/taslp/LiuLCTDZZ23} \\
                                    LSAT \citep{DBLP:journals/taslp/WangLZZWCD22} \\
                                    , leaf
                                ]
                            ]
                            [
                                Text Generation Datasets
                                [
                                    LogicInference \citep{DBLP:journals/corr/abs-2203-15099} \\
                                    FOLIO \citep{DBLP:journals/corr/abs-2209-00840} \\
                                    , leaf
                                ]
                            ]
                        ]
                        [
                            Empirical Evaluation
                            [
                                \citet{DBLP:journals/corr/abs-2302-04023} \\
                                \citet{DBLP:journals/corr/abs-2304-03439} \\
                                \citet{DBLP:journals/corr/abs-2306-09841} \\
                                , leaf
                            ]
                        ]
                    ]
                    [
                        Multi-hop Reasoning
                        [
                            Datasets
                            [
                                HotpotQA \citep{DBLP:conf/emnlp/Yang0ZBCSM18} \\
                                HybridQA \citep{DBLP:conf/emnlp/ChenZCXWW20} \\
                                MultiRC \citep{DBLP:conf/naacl/KhashabiCRUR18} \\
                                NarrativeQA \citep{DBLP:journals/tacl/KociskySBDHMG18} \\
                                Medhop \citep{DBLP:journals/tacl/WelblSR18} \\
                                Wikihop \citep{DBLP:journals/tacl/WelblSR18} \\
                                , leaf
                            ]
                        ]
                        [
                            Empirical Evaluation
                            [
                                \citet{DBLP:journals/corr/abs-2302-04023} \\
                                \citet{DBLP:journals/corr/abs-2307-09009} \\
                                , leaf
                            ]
                        ]
                    ]
                    [
                        Mathematical Reasoning
                        [
                            Datasets before LLMs
                            [
                                AddSub \citep{DBLP:conf/emnlp/HosseiniHEK14} \\
                                MultiArith \citep{DBLP:conf/emnlp/RoyR15} \\
                                AQUA \citep{DBLP:conf/acl/LingYDB17} \\
                                SVAMP \citep{DBLP:conf/naacl/PatelBG21} \\
                                GSM8K \citep{DBLP:journals/corr/abs-2110-14168} \\
                                , leaf
                            ]
                        ]
                        [
                            Datasets for LLMs
                            [
                                VNHSGE \citep{DBLP:journals/corr/abs-2305-12199} \\
                                MATH\citep{DBLP:conf/nips/HendrycksBKABTS21} \\
                                JEEBench \citep{DBLP:journals/corr/abs-2305-15074} \\
                                MATH 401 \citep{DBLP:journals/corr/abs-2304-02015} \\
                                CMATH \citep{DBLP:journals/corr/abs-2306-16636} \\
                                , leaf
                            ]
                        ]
                        [
                            Evaluation Methods
                            [
                                Chain-of-Thought \citep{DBLP:conf/nips/Wei0SBIXCLZ22} \\
                                Plan-and-Solve Prompting \citep{DBLP:conf/acl/WangXLHLLL23} \\
                                , leaf
                            ]
                        ]
                    ]
                ]
                [
                    Tool Learning
                    [
                        Tool Manipulation
                        [
                            Evaluation for \\
                            Tool-augumented Models
                            [
                                LaMDA \citep{DBLP:journals/corr/abs-2201-08239} \\
                                GeneGPT \citep{DBLP:journals/corr/abs-2304-09667} \\
                                , leaf
                            ]
                        ]
                        [
                            Evaluation for \\
                            Tool-oriented Models
                            [
                                Search Engine
                                [
                                    WebCPM \citep{DBLP:conf/acl/QinCJYLZLHDWXQL23} \\
                                    , leaf
                                ]
                            ]
                            [
                                Onlineshopping
                                [
                                    WebShop \citep{DBLP:conf/nips/Yao0YN22} \\
                                    , leaf
                                ]
                            ]
                            [
                                Code Generation
                                [
                                    RoboCodeGen \citep{DBLP:conf/icra/LiangHXXHIFZ23} \\
                                    , leaf
                                ]
                            ]
                            [
                                Robotic Tasks
                                [
                                    ALFWorld \citep{DBLP:conf/iclr/ShridharYCBTH21} \\
                                    ALFRED \citep{DBLP:conf/cvpr/ShridharTGBHMZF20} \\
                                    SayCan \citep{DBLP:conf/corl/IchterBCFHHHIIJ22} \\
                                    Behavior \citep{DBLP:conf/corl/Srivastava0LMXV21} \\
                                    Inner Monologue \citep{DBLP:conf/corl/HuangXXCLFZTMCS22} \\
                                    , leaf
                                ]
                            ]
                        ]
                        [
                            Multi-tool Benchmark
                            [
                                API-Bank \citep{DBLP:journals/corr/abs-2304-08244} \\
                                APIBench \citep{DBLP:journals/corr/abs-2305-15334} \\
                                ToolBench \citep{DBLP:journals/corr/abs-2305-16504} \\
                                ToolAlpaca \citep{DBLP:journals/corr/abs-2306-05301} \\
                                TPTU \citep{DBLP:journals/corr/abs-2308-03427} \\
                                ToolQA \citep{DBLP:journals/corr/abs-2306-13304} \\
                                \citet{DBLP:journals/corr/abs-2304-08354} \\
                                ToolLLM \citep{DBLP:journals/corr/abs-2307-16789} \\
                                RestBench \citep{DBLP:journals/corr/abs-2306-06624} \\
                                , leaf
                            ]
                        ]
                    ]
                    [
                        Tool Creation
                        [
                            \citet{DBLP:journals/corr/abs-2305-17126} \\
                            CREATOR \citep{DBLP:journals/corr/abs-2305-14318} \\
                            , leaf
                        ]
                    ]
                ]
            ]
        \end{forest}
    }
    \caption{An overview of studies on knowledge and capability evaluation for LLMs.}
    \label{fig:knowledge_and_capability_evaluation}
\end{figure*}


==> taxonomies/safety_evaluation.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=hidden-pink!80, text=black, align=center,font=\normalsize,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
]
\begin{figure*}[t!]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=center,
                font=\large,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=center,
                text centered,
                minimum width=5em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=8em,font=\normalsize,}{},
            where level=2{text width=10em,font=\normalsize,}{},
            where level=3{text width=18em,font=\normalsize,}{},
            where level=4{text width=10em,font=\normalsize,}{},
            [
                Safety \\ Evaluation
                [
                    Robustness \\ Evaluation
                    [
                        Prompt \\ Robustness
                        [
                            PromptBench \citep{DBLP:journals/corr/abs-2306-04528} \\ Trustworthy LLMs \citep{DBLP:journals/corr/abs-2308-05374} \\
                            , leaf
                        ]
                    ]
                    [
                        Task \\ Robustness
                        [
                            \citet{DBLP:journals/corr/abs-2302-12095} \\
                            \citet{DBLP:journals/corr/abs-2301-08745} \\
                            \citet{DBLP:journals/corr/abs-2305-11334} \\
                            RobuT \citep{DBLP:conf/acl/ZhaoZNQZTMR23} \\
                            SynTextBench \citep{ko2023robustness} \\
                            \citet{DBLP:journals/corr/abs-2305-08714} \\
                            ReCode \citep{DBLP:conf/acl/0002LQYWSKTRBNR23} \\
                            \citet{DBLP:journals/corr/abs-2306-14583} \\
                            \citet{DBLP:conf/acl/StolfoJSSS23} \\
                            DGSlow \citep{DBLP:conf/acl/LiLGL23} \\
                            \citet{DBLP:conf/eacl/SticklandSKMH23}
                            , leaf
                        ]
                    ]
                    [
                        Alignment \\ Robustness
                        [
                            \citet{DBLP:journals/corr/abs-2305-13860} \\
                            Jailbroken \citep{DBLP:journals/corr/abs-2307-02483} \\
                            MasterKey \citep{DBLP:journals/corr/abs-2307-08715}
                            , leaf
                        ]
                    ]
                ]
                [
                    Risk \\ Evaluation
                    [
                        Evaluating LLMs\\ behaviors
                        [
                            \citet{DBLP:conf/acl/PerezRLNCHPOKKJ23} \\ \citet{DBLP:journals/corr/abs-2306-09983} \\ 
                            BigToM \citep{DBLP:journals/corr/abs-2306-15448} \\ \citet{DBLP:journals/corr/abs-2307-08678} \\
                            \citet{DBLP:journals/corr/abs-2303-13360} 
                            , leaf
                        ]
                    ]
                    [
                        Evaluating LLMs\\ as Agents
                        [
                            AgentBench \citep{liu2023agentbench} \\ 
                            WebArena \citep{DBLP:journals/corr/abs-2307-13854} \\
                            \citet{DBLP:journals/corr/abs-2305-16960} \\
                            \citet{lin2023agentsims} \\
                            \citet{DBLP:journals/corr/abs-2305-15324} \\
                            \citet{satoevaluating}
                            , leaf
                        ]
                    ]
                ]
            ] 
        \end{forest}
    }
    \caption{Overview of safety evaluations for LLMs.}
    \label{fig:safety_evaluation}
\end{figure*}

==> taxonomies/specialized_llm_evaluation.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=hidden-pink!80, text=black, align=center,font=\normalsize,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
]
\begin{figure*}[t!]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=center,
                font=\large,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=center,
                text centered,
                minimum width=5em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=8em,font=\normalsize,}{},
            where level=2{text width=10em,font=\normalsize,}{},
            where level=3{text width=21em,font=\normalsize,}{},
            % where level=4{text width=10em,font=\normalsize,}{},
            [
                \textbf{Specialized LLMs Evaluation}
                [
                    Biology \\
                    and \\
                    Medicine
                    [
                        Medical Exam
                        [
                            \cite{DBLP:journals/corr/abs-2212-13138} \\ \cite{DBLP:journals/corr/abs-2305-09617} \\
                            \cite{DBLP:journals/corr/abs-2207-08143} \\
                            \cite{DBLP:journals/corr/abs-2303-13375} \\
                            %Performance of ChatGPT on USMLE
                            \cite{DBLP:journals/corr/abs-2307-00112} \\
                            %Evaluating the performance of chatgpt in ophthalmology
                            \cite{ANTAKI2023100324} \\
                            % Chatgpt goes to the operating room
                            \cite{oh2023chatgpt}
                            , leaf
                        ]
                    ]
                    [
                        Evaluation in \\
                        Application \\
                        Scenarios
                        [
                            PubMedQA \citep{DBLP:conf/emnlp/JinDLCL19} \\
                            \cite{DBLP:conf/trec/AbachaAPD17} \\
                            \cite{DBLP:journals/corr/abs-2212-13138} \\
                            \cite{10.1001/jamainternmed.2023.1838} \\
                            CLUE \citep{DBLP:journals/corr/abs-2209-14377} \\
                            \cite{tang2023evaluating} \\
                            \cite{Levine2023.01.30.23285067}
                            , leaf
                        ]
                    ]
                    [
                        Evaluation by Human
                        [
                            \cite{DBLP:journals/corr/abs-2212-13138} \\
                            \cite{DBLP:journals/corr/abs-2305-09617}
                            , leaf
                        ]
                    ]
                ]
                [
                    Education
                    [
                        Teaching
                        [
                            \cite{DBLP:journals/corr/abs-2205-07540} \\ \cite{DBLP:conf/bea/WangD23} 
                            , leaf
                        ]
                    ]
                    [
                        Learning
                        [
                            \cite{DBLP:journals/corr/abs-2302-06871} \\ \cite{dai_lin_jin_li_tsai_gasevic_chen_2023}
                            , leaf
                        ]
                    ]
                ]
                [
                    Legislation
                    [
                        Legislation Exam
                        [
                            \cite{bommarito2022gpt} \\
                            \cite{katz2023gpt} \\
                            \cite{choi2023chatgpt} 
                            , leaf
                        ]
                    ]
                    [
                        Legal Reasoning
                        [
                            \cite{DBLP:journals/corr/abs-2212-01326} \\
                            \cite{DBLP:conf/icail/Blair-StanekHD23} \\
                            \cite{DBLP:conf/iclp/NguyenGTSS23}
                            , leaf
                        ]
                    ]
                    [
                        Evaluation in\\
                        Application
                        [
                            \cite{DBLP:journals/corr/abs-2306-09525} \\
                            \cite{DBLP:conf/icail/DeroyG023}
                            , leaf
                        ]
                    ]
                ]
                [
                    Computer Science
                    [
                        Code Generation\\
                        Evaluation
                        [
                            \cite{liu2023your} \\
                            \cite{thapa2022transformer} \\
                            \cite{xu2022systematic}
                            , leaf
                        ]
                    ]
                    [
                        Programming \\
                        Assistance  Evaluation
                        [
                            \cite{leinonen2023comparing} \\
                            \cite{sandoval2023lost} \\
                            \cite{ross2023programmer}
                            , leaf
                        ]
                    ]
                ]
                [
                    Finance
                    [
                        Financial Application
                        [
                             XuanYuan 2.0 \citep{zhang2023xuanyuan} \\
                            FinBERT \citep{araci2019finbert} \\
                            \cite{son2023beyond}
                            , leaf
                        ]
                    ]
                    [
                        Evaluating GPT
                        [
                            \cite{son2023beyond} \\
                            \cite{zaremba2023chatgpt} \\
                            \cite{niszczota2023gpt}
                            , leaf
                        ]
                    ]
                ]
            ] 
        \end{forest}
    }
    \caption{Overview of specialized LLMs evaluation.}
    \label{fig:specialized_LLMs_evaluation}
\end{figure*}
